Tension Estimation and Localization for a Tethered Micro Aerial Robot

This work focuses on the study of tethered fights of a micro quadcopter, with the aim of supplying continuous power to a small-sized aerial robot. Multiple features for facilitating the interaction between a tethered micro quadcopter and a ground base are described in this paper. Firstly, a tether model based on the catenary curve is presented that describes a quadcopter tethered to a point in space. Furthermore, a method capable of estimating the tension applied to the quadcopter, based only on the inertial information from the IMU sensors and the motor thrusts, is presented. Finally, a novel method for localizing the quadcopter by exploiting the tension imposed by the tether and the shape of the tether is described. The proposed methods are evaluated both in simulation and in real world prototype.

==> following.tex <==
\section{Tension Following}
\subsection{Kalman Filter - Filtering using a constant Model}
\label{sec:filtering_const}
The tension that is applied to the quadcopter is applied through human interaction. Given that, the modeling of the system is quite complicated, since the applied tension depends on the intensity of the force that the person makes while pulling the tether. This situation means infinite possibilities for the way that the wire is pulled. The implemented solution considers a model where the tension remains the same, which is almost valid if the wire is not abruptly pulled. Moreover, this model perfectly matches the cases where the tension applied to the quadcopter is due to a mass attached to it, allowing to compute the weight of that mass. 
\par
Consider now that the state ($\hat{x_k}$) is a $\Re^3$ vector (including the tension along $x$, $y$ and $z$ direction) and that $y_k$ is the observation vector, which includes the tension measurements. The observation vector is computed through indirect measurements, using the inertial information from the quadcopter. The state and the observation vector as well as $A$, $B$, $C$ and $D$ matrices are represented in \ref{eq:Kalman_vars}.
\begin{equation}
\label{eq:Kalman_vars}
    \begin{matrix}
        \hat{x}_k=
    \end{matrix}
    \begin{bmatrix}
        Tx_k \\
        Ty_k \\
        Tz_k \\
    \end{bmatrix}
    y_k=
    \begin{bmatrix}
        Tx_k^{obs} \\
        Ty_k^{obs} \\
        Tz_k^{obs} \\
    \end{bmatrix}
    A=C=\begin{bmatrix}
        1 & 0 & 0 \\
        0 & 1 & 0 \\
        0 & 0 & 1 \\
    \end{bmatrix}
    B=D=0
\end{equation}
The tension measurements $T^{obs}$ are obtained through equation \ref{eq:NE_tether}, by replacing its parameters with the sensor readings.
\begin{equation}
\label{eq:NE_tether}
        T^{obs}=m(\Vec{a}+g\Vec{a_3})-R(\eta)F_p + F_{ext}
\end{equation}
Figure \ref{fig:tensionX_all} presents the estimate of the tensions after and before the Kalman filter.
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Images/Tens_following/tensionX_n0_02_all.jpg}
    \caption{Noisy measurements from the sensors, the tension's true value and the estimated tension}
    \label{fig:tensionX_all}
\end{figure}
The tension estimated along $y$ and $z$ have their values around zero while the tension along $x$ converges to -0.02N after the time instant $t=150s$. The Kalman filter has a significant impact on reducing the tension's noise, since its variance is quite low when compared to the values obtained before the Kalman filtering. However, the model used for this problem assumes that the tension between two time instants is constant, which models the system correctly when there is no change on the tension applied, but, introduces a delay when abrupt changes (such as the step signal) are applied.
\par
\bigskip
\textbf{Vertical tension estimation}
\par
The ground-truth value of the vertical tension is calculated through the weight per length unit of the tether, and through the height of the quadcopter. Moreover, the estimated tension is similarly computed as in the simulation results, according to equation \ref{eq:exp_Tv}, in which the term $a_z$ includes the gravitational acceleration.
\begin{equation}
\label{eq:exp_Tv}
    T_v=mass.a_z-cos(\theta).cos(\phi).F_p
\end{equation}
Additionally, equation \ref{eq:exp_Tv} assumes that the  acceleration term $a_z$ is regarding the world frame. However, the acceleration values are provided by the IMU sensor, and so they do not have their representation in the world frame but, instead, in the inertial frame. Given that, it is necessary to apply to the accelerations from the IMU the rotation responsible for the transformation between the inertial and the world frame. Aiming that, equation \ref{eq:aItoaW} presents the expression for the term $a_z$, where the accelerations in the inertial frame along $x$, $y$ and $z$ are denoted by $aI_x$, $aI_y$ and $aI_z$, respectively.
\begin{equation}
    \label{eq:aItoaW}
    a_z=-sin(\phi).aI_x+cos(\phi).sin(\theta).aI_y+cos(\phi).cos(\theta).aI_z
\end{equation}
\par
\bigskip
\textbf{Horizontal tension estimation}
The ground-truth value of the horizontal tension is computed using the weight of a coin that is attached to a wire. Figure \ref{fig:Hor_test_bench} illustrates the scheme of the test-bench used to compute the ground-truth value for the horizontal tension.
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Images/Tens_following/test_bench.png}
    \caption{Test-bench for computing the horizontal tension}
    \label{fig:Hor_test_bench}
\end{figure}
This way, expression \ref{eq:exp_HorGroundThruth} computes the ground-truth value of the horizontal tension, in which T corresponds to the weight of the coin and $\gamma$ is computed according to equation \ref{eq:exp_gamma} - $z_q$ and $z_a$ are the height of the quadcopter and the height of the vertical arm, respectively, and $r_q$ is the quadcopter's radial coordinate assuming the inertial frame presented in figure \ref{fig:Hor_test_bench}.
\begin{equation}
    \label{eq:exp_HorGroundThruth}
    T_0=cos(\gamma).T
\end{equation}
\begin{equation}
\label{eq:exp_gamma}
    \gamma=tan^-1(\frac{z_q-z_a}{r_q})
\end{equation}
By using the quadcopter's attitude and the total thrust produced by the motors, equation \ref{eq:exp_Tx} and \ref{eq:exp_Ty} calculate the tension along $x$ and $y$, respectively.
\begin{equation}
    \label{eq:exp_Tx}
    T_x=-[sin(\psi).sin(\theta)+cos(\psi).sin(\phi).cos(\theta)].F_p
\end{equation}
\begin{equation}
    \label{eq:exp_Ty}
    T_y=[cos(\psi).sin(\theta)-sin(\psi).sin(\phi).cos(\theta)].F_p
\end{equation}
Firstly, it is used a coin of 1 cent - with a weight of 2,3g - attached to the quadcopter through a linen wire, with negligible mass and contact force. Figure \ref{fig:Hor_sfio} illustrates the estimated horizontal tension and its ground-truth value, computed according to equation \ref{eq:exp_HorGroundThruth}.
\begin{figure}[H]
    \centering     
    \subfigure[Horizontal tension test one]{
        \includegraphics[width=0.45\linewidth]{Images/Tens_following/T0_test1.png}
    }
    \subfigure[Horizontal tension test two]{
        \includegraphics[width=0.45\linewidth]{Images/Tens_following/T0_test2.png}
    }
    \caption{Horizontal tension for $x\simeq-0.4m$, $y\simeq0m$ and $z\simeq1m$, using the untethered - \textbf{Blue} is the ground-truth value for tension $T_0$, \textbf{red} is the estimated tension $T_0$, \textbf{orange} and \textbf{green} are the $T_x$ and $T_y$ tensions}
    \label{fig:Hor_sfio}
\end{figure}
Secondly, the estimation of the horizontal tension is evaluated on the quadcopter that is powered by the silicon wire, and the coin is directly sticked on to the silicon cable. Due to the properties of the silicon material, the contact force of the tether and its weight can no longer be considered negligible. Given that, in order to know the ground-truth value of the coin's impact, i.e., without depending on the silicon tether, two experiments are executed and both assume that the tether's shape is similar between them. The first experiment evaluates the horizontal tension without having the coin attached to the tether, while the second experiment estimates the horizontal tension having the coin attached. This way, the ground-truth of the horizontal tension in the second experiment is the sum of the horizontal tension estimate concerning the first experiment with the coin's weight. Figure \ref{fig:Hor_cfio} displays the estimate of the horizontal tension, as well as its ground-truth value regarding a position of $x\simeq-0,3m$ and $y\simeq0m$
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth
    ]{Images/Tens_following/T0_cM&fio.png}
    \caption{Horizontal tension for $x\simeq-0.4m$, $y\simeq0m$ and $z\simeq1m$, using the tethered quadcopter - \textbf{Blue} is the ground-truth value for tension $T_0$, \textbf{red} is the estimated tension $T_0$, \textbf{orange} and \textbf{green} are the $T_x$ and $T_y$ tensions}
    \label{fig:Hor_cfio}
\end{figure}
The process of estimating the ground-truth value of the horizontal tension using the previously mentioned test-bench hampers to get accurate values of the ground-truth. Given that, in section \ref{sec:pos_est}, the accuracy of the tension's estimate is indirectly evaluated for more case scenarios. Since the position's estimation is directly related with estimation of the tension, evaluating the accuracy of the position's estimation is also evaluating, in an indirect way, the accuracy of the tension's estimate.
\par
At last, it is also ensured that the horizontal tension for a vertical flight (a flight where the tether direction is mainly vertical) is nearly null - less than 0.01N - (see figure \ref{fig:Hor_vert1m}). Such test does not require any test-bench, as opposed to the previous experiments
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Images/Tens_following/T0_v03m.png}
    \caption{Horizontal tension of a hovering flight with position $x=0$, $y=0$ and $z=0$ - \textbf{blue} and \textbf{yellow} are the tension $T_x$ and $T_y$, \textbf{green} is the tension $T_0$}
    \label{fig:Hor_vert1m}
\end{figure}
%%%%%%%%%%%%%%%%
\subsection{Kalman Filter - Filtering using a non-constant model}
In section \ref{sec:filtering_const}, the Kalman filter models the tension of the tether as being constant, which is valid for the hovering case. However, it initially seems inappropriate to use it when modeling a tension that is, for sure, not constant. As an approach to this reality, it is implemented a model that takes into account the first and the second derivatives, in order to predict the pulling movement that may be applied. To simplify the development of the model, without loss of generality, consider only the tension along the $x$ direction. Assume that equation \ref{eq:kalman_alternative} defines the Kalman model in discrete time.
\begin{equation}
\label{eq:kalman_alternative}
    Tx_{k+1}=Tx_k+a(Tx_k-Tx_{k-1})+b(Tx_k-Tx_{k-1}-(Tx_{k-1}-Tx_{k-2}))
\end{equation}
Figure \ref{eq:state_space_alt} represents the state space derived from the equation \ref{eq:kalman_alternative}.
\begin{equation}
\label{eq:state_space_alt}
    \begin{bmatrix}
    x_{1[k+1]} \\
    x_{2[k+1]} \\
    x_{3[k+1]} \\
    \end{bmatrix}
    =
    \begin{bmatrix}
    0 && 1 && 0 \\
    0 && 0 && 1 \\
    b && -(a+2b) && (1+a+b)
    \end{bmatrix}
    \begin{bmatrix}
    x_{1[k]} \\
    x_{2[k]} \\
    x_{3[k]} \\
    \end{bmatrix}
\end{equation}
The state $x_{3[k]}$,$x_{2[k]}$ and $x_{1[k]}$ corresponds to the tension $Tx_k$, $Tx_{k-1}$ and $Tx_{k-2}$, respectively, and the parameters $a$ and $b$ represent the weight given to each derivative.
\par
The performance of these two models is tested in Matlab for the case where the applied tension is a step signal, but without considering the drag effect. The parameters use the values $a=0.978, b=-0.97$ and figure \ref{fig:diff_aproaches} displays the results.
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Images/Tens_following/diff_aproaches(2).jpg}
    \caption{Real tension (pink), tension estimated using the constant model (green) and tension estimated using the derivative model (yellow)}
    \label{fig:diff_aproaches}
\end{figure}
As it can be observed the new model presents slight improvements, since it can converge faster to the real value and it also presents less noise for the steady values, as illustrated in figure \ref{fig:diff_aproaches2nd}.
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Images/Tens_following/diff_aproaches(1).jpg}
    \caption{Zoom of figure \ref{fig:diff_aproaches}}
    \label{fig:diff_aproaches2nd}
\end{figure}
These results may look contradictory since the initial model is ideally "perfect" for modeling constant values. However, this new model allows to increase the confidence in the model (by decreasing the noise variance of process), making it less susceptible to the observation noise without losing the ability of following fast changes.
%%%%%%%%%%%%%%%%%%
\subsection{Tension following by maintaining a null tension applied to the UAV}
In the previous section the quadcopter's position is updated if the estimated tension is greater than a pre-defined threshold. This means that it is necessary to know the quadcopter's current position, which implies the use of an external system such as the Mocap system. An alternative way is to assume that the tether outlines a catenary curve and that the outer loop controller no longer uses the goal and the current position (as in figure \ref{fig:cascade}) but, instead, uses a goal tension and a current tension (see figure \ref{fig:controller2}). 
\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{Images/Tens_following/Controller2.png}
    \caption{Control Structure}
    \label{fig:controller2}
\end{figure}
The quadcopter's current tension is estimated during flight as shown before, using the attitude, thrust and acceleration of the quadcopter. The goal tension is computed by providing a goal position, regarding the tether's frame, and using the catenary's properties to compute the goal tension according to a perfect catenary.
\par
Figure \ref{fig:tf_sim_result} presents the simulation results obtained using the strategy previously described. However, due to the inaccurate estimation of the vertical tension in the initial instants, the quadcopter's feedback loop of the altitude uses the altitude values - the goal and the current altitude - instead of using the values of the vertical tension. In practice, the altitude can be computed using a distance sensor or, for cases of higher altitudes, by using an altimeter sensor.   
\begin{figure}[H]
    \centering
    \subfigure[Flight test one]{
        \includegraphics[width=0.45\linewidth]{Images/Tens_following/tens_foll1.jpg}
    }
    \subfigure[Flight test two]{
        \includegraphics[width=0.45\linewidth]{Images/Tens_following/tens_foll2.jpg}
    }
    \caption{Simulation results of the goal and current position along $x$, $y$ and $z$}
    \label{fig:tf_sim_result}
\end{figure}
\subsection{Tension following by position updating}
To observe in real life the behaviour of the \textbf{tension following} solution a few videos are taken \footnote{The full videos are presented on Youtube at . . . }, where figure \ref{fig:tens_foll_vid1} corresponds to screenshots of one of these videos.
\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{Images/Tens_following/tens_foll_vid1.jpg}
    \caption{Screenshots of the quadcopter following the tension's direction}
    \label{fig:tens_foll_vid1}
\end{figure}
Moreover, the implementation of the \textbf{tension following} feature can also be used for the landing process. Given that, after the first pull, a flag is activated indicating that the tension following feature is on. After that, if the quadcopter flies under a certain height, the motors are turned off. Without using an external motion system, the same principle can be applied using a sensor distance, which deactivates the motors if the distance to the landing platform is smaller than a threshold. Figure \ref{fig:tens_foll_vid2} illustrates the landing process mentioned before.
\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{Images/Tens_following/tens_foll_vid2.jpg}
    \caption{Screenshots of the landing of the quadcopter using the \textbf{tension following} feature}
    \label{fig:tens_foll_vid2}
\end{figure}
